Multiple Coulomb Scattering of muons in Lithium Hydride

Multiple Coulomb Scattering (MCS) is a well known phenomenon occurring when charged particles traverse materials. Measurements of muons traversing low $Z$ materials made in the MuScat experiment showed that theoretical models and simulation codes, such as GEANT4 (v7.0), over-estimated the scattering. The Muon Ionization Cooling Experiment (MICE) measured the cooling of a muon beam traversing a liquid hydrogen or lithium hydride (LiH) energy absorber as part of a programme to develop muon accelerator facilities, such as a Neutrino Factory or a Muon Collider. The energy loss and MCS that occur in the absorber material are competing effects that alter the performance of the cooling channel. Therefore measurements of MCS are required in order to validate the simulations used to predict the cooling performance in future accelerator facilities. We report measurements made in the MICE apparatus of MCS using a LiH absorber and muons within the momentum range 160 to 245 MeV/c. The measured RMS scattering width is about 9% smaller than that predicted by the approximate formula proposed by the Particle Data Group. Data at 172, 200 and 240 MeV/c are compared to the GEANT4 (v9.6) default scattering model. These measurements show agreement with this more recent GEANT4 (v9.6) version over the range of incident muon momenta.

==> AuthorList.tex <==
%======= Author list: 2021, System performance paper
%

\thispagestyle{plain}
\setlength\parindent{0em}%\noindent

\section{The MICE collaboration}

\author{M.~Bogomilov,  R.~Tsenov, G.~Vankova-Kirilova}
\affiliation{
Department of Atomic Physics, St.~Kliment Ohridski University of Sofia, 5 James Bourchier Blvd, Sofia, Bulgaria
}

\author{Y.~P.~Song, J.~Y.~Tang}
\affiliation{
Institute of High Energy Physics, Chinese Academy of Sciences, 19 Yuquan Rd, Shijingshan District, Beijing, China
}

\author{Z.~H.~Li}
\affiliation{
Sichuan University, 252 Shuncheng St, Chengdu, China
}

\author{R.~Bertoni, M.~Bonesini, F.~Chignoli, R.~Mazza}
\affiliation{
Sezione INFN Milano Bicocca and Dipartimento di Fisica G.~Occhialini, Piazza della Scienza 3, Milano, Italy
}


\author{V.~Palladino}
\affiliation{
Sezione INFN Napoli and Dipartimento di Fisica, Universit\`{a} Federico II, Complesso Universitario di Monte S.~Angelo, via Cintia, Napoli, Italy
}

\author{A.~de Bari}
\affiliation{ 
Sezione INFN Pavia and Dipartimento di Fisica, Universit\`{a} di Pavia, Via Agostino Bassi 6, Pavia, Italy
}

\author{D.~Orestano, L.~Tortora}
\affiliation{
Sezione INFN Roma Tre and Dipartimento di Matematica e Fisica, Universit\`{a} Roma Tre, Via della Vasca Navale 84, Roma, Italy
}

\author{Y.~Kuno, H.~Sakamoto\footnote{Current address RIKEN 2-1 Hirosawa, Wako, Saitama, Japan}, A.~Sato}
\affiliation{
Osaka University, Graduate School of Science, Department of Physics, 1-1 Machikaneyamacho, Toyonaka, Osaka, Japan
}

\author{S.~Ishimoto}
\affiliation{
High Energy Accelerator Research Organization (KEK), Institute of Particle and Nuclear Studies, Tsukuba, Ibaraki, Japan
}


\author{M.~Chung, C.~K.~Sung}
\affiliation{ 
Department of Physics, UNIST, 50 UNIST-gil, Ulsan, South Korea
}

\author{F.~Filthaut\footnote{Also at Radboud University, Houtlaan 4, Nijmegen, Netherlands}}
\affiliation{
Nikhef, Science Park 105, Amsterdam, Netherlands
}

\author{M.~Fedorov}
\affiliation{
Radboud University, Houtlaan 4, Nijmegen, Netherlands
}

\author{D.~Jokovic, D.~Maletic, M.~Savic}
\affiliation{
Institute of Physics, University of Belgrade, Serbia
}

%\newpage

\author{N.~Jovancevic, J.~Nikolov}
\affiliation{
Faculty of Sciences, University of Novi Sad, Trg Dositeja Obradovi\'{c}a 3, Novi Sad, Serbia
}

\author{M. ~Vretenar, S.~Ramberger}
\affiliation{
CERN, Esplanade des Particules 1, Geneva, Switzerland
}

\author{R.~Asfandiyarov, A.~Blondel, F.~Drielsma\footnote{Current address SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, California, USA}, Y.~Karadzhov }
\affiliation{
DPNC, Section de Physique, Universit\'e de Gen\`eve, 24 Quai Ernest-Ansermet, Geneva, Switzerland
}

\author{G.~Charnley, N.~Collomb,  K.~Dumbell, A.~Gallagher, A.~Grant, S.~Griffiths,  T.~Hartnett, B.~Martlew, 
A.~Moss, A.~Muir, I.~Mullacrane, A.~Oates, P.~Owens, G.~Stokes, P.~Warburton, C.~White}
\affiliation{
STFC Daresbury Laboratory, Keckwick Ln, Daresbury, Cheshire, UK
}

\author{D.~Adams,   V.~Bayliss, J.~Boehm, T.~W.~Bradshaw, C.~Brown\footnote{Also at College of Engineering, Design and Physical Sciences, Brunel University, Kingston Lane, Uxbridge, UK}, M.~Courthold,  J.~Govans, M.~Hills, J.-B.~Lagrange, C.~Macwaters, A.~Nichols, R.~Preece, S.~Ricciardi, C.~Rogers, T.~Stanley, J.~Tarrant,  
M.~Tucker, S.~Watson\footnote{Current address ATC, Royal Observatory Edinburgh, Blackford Hill, Edinburgh, UK},A.~Wilson}
\affiliation{
STFC Rutherford Appleton Laboratory, Harwell Campus, Didcot, UK
}

\author{R.~Bayes\footnote{Current address Laurentian University, 935 Ramsey Lake Road, Sudbury, Ontario, Canada},  J.~C.~Nugent, F.~J.~P.~Soler}
\affiliation{
School of Physics and Astronomy, Kelvin Building, University of Glasgow, Glasgow, UK
}

\author{R.~Gamet, P.~Cooke}
\affiliation{
Department of Physics, University of Liverpool, Oxford St, Liverpool, UK
}

\author{V.~J.~Blackmore, D.~Colling, A.~Dobbs\footnote{Current address OPERA Simulation Software, Network House, Langford Locks, Kidlington, UK}, P.~Dornan, P.~Franchini\footnote{Current address Lancaster University, Physics avenue, Lancaster, UK}, C.~Hunt\footnote{Current address CERN, Esplanade des Particules 1, Geneva, Switzerland}, P.~B.~Jurj, A.~Kurup, K.~Long, J.~Martyniak,  S.~Middleton\footnote{Current address School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, UK}, J.~Pasternak, M.~A.~Uchida\footnote{Current address Rutherford Building, Cavendish Laboratory, JJ Thomson Avenue, Cambridge, UK}}
\affiliation{
Department of Physics, Blackett Laboratory, Imperial College London, Exhibition Road, London, UK
}

\author{J.~H.~Cobb}
\affiliation{
Department of Physics, University of Oxford, Denys Wilkinson Building, Keble Rd, Oxford, UK
}

\author{C.~N.~Booth, P.~Hodgson, J.~Langlands, E.~Overton\footnote{Current address Arm, City Gate, 8 St Mary's Gate, Sheffield, UK}, V.~Pec,  P.~J.~Smith, S.~Wilbur}
\affiliation{
Department of Physics and Astronomy, University of Sheffield, Hounsfield Rd, Sheffield, UK
}

\author{G.~T.~Chatzitheodoridis\footnote{Also at School of Physics and Astronomy, Kelvin Building, University of Glasgow, Glasgow, UK}$^,$\footnotemark, A.~J.~Dick\footnotemark[\value{footnote}],  K.~Ronald\footnotemark[\value{footnote}], C.~G.~Whyte\footnotemark[\value{footnote}], A.~R.~Young\footnotemark[\value{footnote}]
\footnotetext{Also at Cockcroft Institute, Daresbury Laboratory, Sci-Tech Daresbury, Keckwick Ln, Daresbury, Warrington, UK}}
\affiliation{
SUPA and the Department of Physics, University of Strathclyde, 107 Rottenrow, Glasgow, UK
}

\author{S.~Boyd,  J.~R.~Greis\footnote{Current address TNG Technology Consulting, Beta-Strasse 13A, Unterf\"{o}hring, Germany}, T.~Lord, C.~Pidcott\footnote{Current address Department of Physics and Astronomy, University of Sheffield, Hounsfield Rd, Sheffield, UK}, I.~Taylor\footnote{Current address Defence Science and Technology Laboratory, Porton Down, Salisbury, UK}}
\affiliation{
Department of Physics, University of Warwick, Gibbet Hill Road, Coventry, UK
}

\author{M.~Ellis\footnote{Current address Macquarie Group, 50 Martin Place, Sydney, Australia}, R.B.S.~Gardener\footnote{Current address Inawisdom, Columba House, Adastral park, Martlesham, Ipswich, UK}, P.~Kyberd, J.~J.~Nebrensky\footnote{Current address UK Atomic Energy Authority, Culham Science Centre, Abingdon, UK}}
\affiliation{
College of Engineering, Design and Physical Sciences, Brunel University, Kingston Lane, Uxbridge, UK
}

\author{M.~Palmer, H.~Witte}
\affiliation{
Brookhaven National Laboratory, 98 Rochester St, Upton, New York, USA
}

\newcounter{FNEuclid}
\author{D.~Adey\footnote{Current address Institute of High Energy Physics, Chinese Academy of Sciences, 19 Yuquan Rd, Shijingshan District, Beijing, China}, A.~D.~Bross, D.~Bowring, P.~Hanlet, A.~Liu\footnotemark\footnotetext{Current address Euclid Techlabs, 367 Remington Blvd, Bolingbrook, Illinois, USA}\setcounter{FNEuclid}{\value{footnote}}, D.~Neuffer, M.~Popovic, P.~Rubinov}
\affiliation{
Fermilab, Kirk Rd and Pine St, Batavia, Illinois, USA
}

\author{A.~DeMello, S.~Gourlay, A.~Lambert, D.~Li, T.~Luo, S.~Prestemon,  S.~Virostek}
\affiliation{
Lawrence Berkeley National Laboratory, 1 Cyclotron Rd, Berkeley, California, USA
}

\author{B.~Freemire\footnotemark[\value{FNEuclid}], D.~M.~Kaplan, T.~A.~Mohayai\footnote{Current address Fermilab, Kirk Rd and Pine St, Batavia, Illinois, USA}, D.~Rajaram\footnote{Current address KLA, 2350 Green Rd, Ann Arbor, Michigan, USA}, P.~Snopok, Y.~Torun}
\affiliation{
Illinois Institute of Technology, 10 West 35th St, Chicago, Illinois, USA
}

\author{L.~M.~Cremaldi, D.~A.~Sanders, D.~J.~Summers\footnote{Deceased}}
\affiliation{
University of Mississippi, University Ave, Oxford, Mississippi, USA
}

\author{L.~R.~Coney\footnote{Current address European Spallation Source ERIC, Partikelgatan 2, Lund, Sweden}, G.~G.~Hanson, C.~Heidt\footnote{Current address Swish Analytics, Oakland, California, USA}}
\affiliation{
University of California, 900 University Ave, Riverside, California, USA
}

